Lemur: Integrating Large Language Models in Automated Program Verification

The demonstrated code-understanding capability of LLMs raises the question of whether they can be used for automated program verification, a task that demands high-level abstract reasoning about program properties that is challenging for verification tools. We propose a general methodology to combine the power of LLMs and automated reasoners for automated program verification. We formally describe this methodology as a set of transition rules and prove its soundness. We instantiate the calculus as a sound automated verification procedure and demonstrate practical improvements on a set of synthetic and competition benchmarks.

==> backup_rebuttal.tex <==
In general, there are several valuable advantages in defining a calculus as it allows to perform theoretical comparisons of different  

Derivation rules enable theoretical analysis of the power of any implementation, like Algorithm 1, including the design of problem families that are either provably hard or easy for this set of rules. For instance, resolution is a set of underlying derivation rules for SAT solvers. It has been proven that resolution cannot solve the Pigeon Hole Problem in polynomial time. Therefore, SAT solvers cannot solve it in poly time (unless they go beyond resolution).

2. In general, proof systems allow for the study and comparison of different proof systems' power. If one comes up with different derivation rules, we can compare them to those in Lemur.

3. It lays the foundation for defining new algorithms that determine alternatives to Alg 1 strategies for rule applications.


    

==> rebutal2.tex <==

Q: Completeness of rules

We strongly disagree that the value of abstract calculus is only the proof of completeness. Many highly impactful abstract calculus in SMT (e.g., notably Model-Constructing Satisfiability Calculus [1]) do not attempt to establish completeness results. In the context of formal methods, abstract calculus has the following benefits:
    A separation between the implementation and the theory
    Highlighting the key features of the procedure in a modular manner
    Provides formalized grounds for future extension.
     
Also, we would like to point out that all SMT solvers, which are the backends of program verifiers, are incomplete for some theories. However, they are very valuable tools for verification and bug finding.

Q: Running program verification performance on a cloud/more resources

We are not aware of any reported significant performance gains in software verification tasks with parallelization. In fact, a very recent paper shows that achieving parallelization of SMT solvers — the underlying solvers for both UAutomizer and ESBMC — is not trivial. For example, using 64 cores resulted in less than 2 times speed-up.  We therefore do not expect that allocating more computational resources to the verifier will significantly improve the number of instances solved within the given time bound.

[1] Partitioning Strategies for Distributed SMT Solving
Amalee Wilson, Andres Noetzli, Andrew Reynolds, Byron Cook, Cesare Tinelli, and Clark Barrett,
FMCAD'23




----------


Q: Running Lemur locally/free

To run Lemur locally, we need to use an open-source model. As our experiments show, even using GPT-3.5 degrades the benefits of synergy between LLM and verification. We do not believe we can obtain better results with open-source models

We note that the cost of calling GPT is not high, only 2 cents per call. For safety-critical applications, such cost is easily justifiable given the potential bug costs




----------------------------
I tend to agree with Reviewer 2ahy's concerns on the fairness of a runtime comparison between the baselines and LEMUR using a LLM oracle running on external hardware. I understand that running the LLM oracle locally is not completely solving the issue, since most reachability tools do not make use of the GPU anyway (to the best of my understanding). Yet, in my opinion having LEMUR running completely on local would be more significant for practitioners, giving some insight on the performance gains that we can expect on limited hardware resource



-------

I believe my comment about abstract rules has been mis-interpreted. Let me clarify. I am well aware of the value of formalization of abstract rules for various algorithms in the area of formal methods. It would be unfair to interpret my comment as saying that the only value of abstract rules in any context is in proving completeness. My comment was in the specific context of Lemur. The algorithm presented by the authors can be proved sound without reference to the rules, in my opinion. So, proving soundness of the algorithm is not a strong value addition (if at all) of the rules. I agree that abstraction of steps allows scope for further generalizations in an elegant way. A sterling example of this is [1], where Simplex was generalized to Reluplex. The paper on model-constructing satisfiability calculus for SMT theories that the authors point out achieves a whole bunch of objectives through the abstract rules: it presents a unifying framework for a large collection of model-based SMT decision procedures, allows DPLL(T) and the nlsat proof calculus to be combined, and also allows a simpler correctness proof than nlsat. I don't see any such value additions of the Lemur proof calculus beyond the correctness proof of the Lemur algorithm, and even there I don't see any simplifications that are obtained by the rule abstraction. I agree that the rules in the case of Lemur provide modular highlighting of features of the algorithm. However, I disagree that in the specific case of Lemur, the rules provide a significant separation between theory and implementation, beyond what the steps of the algorithm already provide. This is why I had commented that a potential value addition of the set of rules in the specific case of Lemur could have been a step towards proving completeness. To interpret this as saying that the only value of rule formalization in all cases is to prove completeness is completely taking my comment out of context.

> We thank the reviewer for their clarifications. We now understand better what is the reviewer's concern regarding the value of the rules in proving soundness of Algorithm 1. 

We agree with the reviewer that one can directly prove the soundness of Algorithm 1. However, if someone proposes an alternative algorithm based on our rules, they have to re-prove soundness.

We chose to prove the soundness of the calculus instead of just Algorithm 1 because this allows us to cover all possible proof derivations, so that any alternative algorithm based on our rules is sound by construction.





Regarding the comment about use of parallelization, I wasn't referring only to parallelization. If we are willing to spend more resources on computing, we might as well use the additional resources to run a tool for longer duration or with more memory than the limits imposed by SV-COMP. Are the authors saying that this doesn't help in improving the tally of verification results? This reviewer has to respectfully disagree, based on first-hand experience. In fact, the paper pointed to by the authors already shows improvement, though not as much as a nicely parallelizable task would show. This just shows that parallelization is difficult, though it does provide improvements. Even if we go by the parallelization results pointed to by the authors, wouldn't a better comparison be to see how ESBMC or UAutomizer fares with the same budget used for GPT calls (as in Lemur) and for additional cores on a cloud platform? Unless we take the cost-benefit analysis of this into account, it may be a bit premature to assert that Lemur helps improve existing tools.

We thank the reviewer for the clarifications. 

Regarding longer timeout, we have run both ESBMC and UAutomizer on the benchmarks with a 1-hour timeout, and no additional instances were solved. While we are happy to report results with a longer timeout in the final version, we believe it will unlikely help in most of these benchmarks, as we observed that the verifiers typically got stuck in the call to the underlying SMT solver.

Regarding parallelization, we agree that the comparison that the reviewer suggested would be an interesting experiment. However, we are not aware of cloud/massively parallel adaptations of ESBMC or UAutomizer that are readily available. Creating efficient massively parallel automated reasoners is a challenging research problem on its own and we believe it is out-of-scope of our work. 



------

Dear Area Chair,  we would like to report that we have addressed all comments of the reviewers. 
There have not been follow-up questions/objections to our latest responses to all reviewers.


*We would like to specifically bring to your attention several Reviewer 2ahy’s points, which 
we find unwarranted for the following reasons*:

1. Reviewer 2ahy requested us to run the baseline verifiers (ESBMC and UAutomizer) in the cloud with the same budget as Lemur to have an apple-to-apple comparison of computational resources.
Unfortunately, **this request is unrealistic** for two reasons: First, neither solver is cloud-based or massively parallelizable. In fact, *we are not aware of any software verifiers of this nature, and neither did Reviewer 2ahy provide any references*. Second, effective parallelization of verification tools is known to be an *open challenge* that the formal methods community is actively working on. 
We also note the fact that we found a way to utilize massive computational resources, including GPUs, to accelerate the verifiers is highly non-trivial and has a lot of potential.


2. Reviewer 2ahy also notes that our Lemur implementation uses paid OpenAI API services, i.e. GPT-family LLMs, which hampers reproducibility and usability. First, we have noted that we will make our implementation publicly available for the community to reproduce our results. Second, **our rationale for using SoTA LLMs is that we want to investigate the full potential of the proposed methodology**, and, as the performance of open-source LLMs keeps improving, Lemur can be effectively instantiated with open-source models in the future.


3. Finally, Reviewer 2ahy questions the necessity of our presentation of Lemur as an abstract calculus. 
As authors, we believe the calculus laid out a formal foundation for the integration of LLMs and automated reasoners, and is an important part of the paper. We also note this separation between theory and implementation is a very standard practice in formal methods (e.g., [1, 2, 3]). 
*Please note that our calculus already triggered constructive discussions with reviewer mzY5*.

We thank you for your attention, and sincerely wish you could please take this feedback into consideration!

[1] Solving SAT and SAT Modulo Theories. Robert Nieuwenhuis, Albert Oliveras,and Cesare Tinelli.  Journal of the ACM (2006).
[2] A decision procedure for an extensional theory of arrays. Aaron Stump, Clark W. Barrett, David L. Dill, and Jeremy Levitt. LICS (2001).
[3] Decision Procedures for Algebraic Data Types with Abstractions. Philippe Suter, Mirco Dotta, and Viktor Kuncak. POPL (2010).
